Privacy Law Enforcement Under Centralized Governance: A Qualitative Analysis of Four Years' Special Privacy Rectification Campaigns

In recent years, major privacy laws like the GDPR have brought about positive changes. However, challenges remain in enforcing the laws, particularly due to under-resourced regulators facing a large number of potential privacy-violating software applications (apps) and the high costs of investigating them. Since 2019, China has launched a series of privacy enforcement campaigns known as Special Privacy Rectification Campaigns (SPRCs) to address widespread privacy violations in its mobile application (app) ecosystem. Unlike the enforcement of the GDPR, SPRCs are characterized by large-scale privacy reviews and strict sanctions, under the strong control of central authorities. In SPRCs, central government authorities issue administrative orders to mobilize various resources for market-wide privacy reviews of mobile apps. They enforce strict sanctions by requiring privacy-violating apps to rectify issues within a short timeframe or face removal from app stores. While there are a few reports on SPRCs, the effectiveness and potential problems of this campaign-style privacy enforcement approach remain unclear to the community. In this study, we conducted 18 semi-structured interviews with app-related engineers involved in SPRCs to better understand the campaign-style privacy enforcement. Based on the interviews, we reported our findings on a variety of aspects of SPRCs, such as the processes that app engineers regularly follow to achieve privacy compliance in SPRCs, the challenges they encounter, the solutions they adopt to address these challenges, and the impacts of SPRCs, etc. We found that app engineers face a series of challenges in achieving privacy compliance in their apps...

==> sections/old_background.tex <==
\section{Background}
\label{sec:background}

\subsection{Enforcement of EU Privacy Laws} 
%
The General Data Protection Regulation (GDPR), enforced by the EU Parliament on May 25, 2018, is widely recognized as a comprehensive law safeguarding individuals' privacy rights.
%
It establishes a legal framework for the autonomous enforcement of general privacy principles by supervisory agencies, specifically Data Protection Authorities (DPAs), distributed across various EU member states.
%
DPAs typically identify potential GDPR violations through privacy complaints from individuals or by monitoring public industry reports. Then, they investigate the involved organizations (or data controllers) to determine if the organizations are indeed violating GDPR,  by gathering evidence, conducting interviews, and assessing organizational activities.
%
DPAs have the authority to request organizations to rectify their privacy practices or impose fines for violations. In many cases, they disclose information about the violations (and the fines) to raise awareness among the public and other organizations.

Such enforcement practices, characterized by 1) \textit{being primarily driven by complaints and industry reports}~\cite{saemann2022investigating} and 2) \textit{being supported by autonomous actions of supervisory agencies under the guidance of general privacy laws}, represent a common approach to enforcing various other privacy laws including the US federal and state laws. 
%




\jingtao{
\subsection{Enforcement of US Privacy Laws} 
\ignore{For example, the enforcement of Children's Online Privacy Protection Act (COPPA)~\cite{coppa} by the Federal Trade Commission (FTC)~\cite{ftc}, and the enforcement of the California state law, the California Consumer Privacy Act (CCPA)~\cite{ccpa}, by the California Attorney General's office~\cite{cagoffice}.}
% \subsection{Enforcement of US Privacy Laws} 
%
%不同于欧洲建立的统一的GDPR，美国的privacy laws是decentralized且fragmented。
% 这些隐私法律都是针对于国家不同事务、地域、管理机构等而设立的sector-specific，例如，联邦贸易委员会（FTC）执行《儿童在线隐私保护法案》（COPPA），以及加州总检察长办公室执行加州法律《加州消费者隐私法案》（CCPA）。
% 与之相对应，美国并没有一个统一的隐私法律的执法机构，而是结合国家中的不同sector，如美国联邦贸易委员会、州检察长、证券交易委员会、消费者金融保护局、美国联邦贸易委员会（FTC）等各自成为隐私法律的执法机构。
Unlike the unified GDPR established in Europe, privacy laws in the United States are decentralized and fragmented. These privacy laws are designed for specific sectors related to national affairs, regions, and regulatory bodies. 
%
% For example, the Federal Trade Commission (FTC) enforces the Children's Online Privacy Protection Act (COPPA), and the California Attorney General's Office enforces the California Consumer Privacy Act (CCPA). In contrast, the United States does not have a unified enforcement agency for privacy laws. 
For example, the enforcement of Children's Online Privacy Protection Act (COPPA)~\cite{coppa} by the Federal Trade Commission (FTC)~\cite{ftc}, and the enforcement of the California state law, the California Consumer Privacy Act (CCPA)~\cite{ccpa}, by the California Attorney General's office~\cite{cagoffice}.
%
Instead, different sectors within the country, such as the Federal Trade Commission, state attorneys general, the Securities and Exchange Commission, the Consumer Financial Protection Bureau, and others, each serve as enforcement agencies for privacy laws.
%
}


\TODO{Large-scale privacy enforcement campaign with strong government control.}
\url{https://papers.ssrn.com/sol3/papers.cfm?abstract\_id=3827228, https://elibrary.law.psu.edu/cgi/viewcontent.cgi?article=1244&context=jlia}
% maintain strong government control and public order

\subsection{Enforcement of Chinese Privacy Laws}
\label{subsec:background_chinese}
The enforcement of Chinese privacy laws differs from GDPR and US laws due to the unique hierarchy of privacy laws, provisions, and guidelines\ignore{ guidelines, and specifications}, along with the proactive enforcement campaigns launched by government agencies.

\para{Chinese privacy laws, provisions, and guidelines}
%
In the past decade, the National People's Congress of China has enacted a series of laws and regulations that protect data security and privacy, such as the Cybersecurity Law (2016)\cite{cybersecuritylaw}, the Regulations on Telecommunications (2000)~\cite{regulationsontelecommunications}, and the Personal Information Protection Law (PIPL, 2021)\cite{pipl}, etc.
%
These laws outline a series of general privacy principles in a way very similar to GDPR. 

% 不同于西方国家，中国对隐私数据的保护来源于保卫国家的cyber-Sovereignty。在中国政府看来，国家cyber-Sovereignty的重要性与公民个人的隐私保护是同等重要的。在中国，对于隐私法律的执行需要中国政府保持强有力的控制和社会秩序。出于对国家网络安全和公民个人信息保护的考量，中国政府会主动要求并且监督公司遵守隐私法律，这区别于欧洲GDPR执行过程中由用户发起的对公司隐私数据保护的监管。而这种由中国政府主导的top-to-down式的隐私法律执行，也不同于美国decentralized式的隐私法律执行。
\jingtao{
Unlike Western countries, China's protection of privacy data originates from the defense of national cyber-Sovereignty. In the eyes of the Chinese government, the importance of national cyber-Sovereignty is on par with the protection of individual citizens' privacy. 
% 
In China, the enforcement of privacy laws requires the Chinese government to maintain strong control and social order. Out of consideration for national cyber security and the protection of citizens' personal information, the Chinese government actively requires and supervises companies to comply with privacy laws, which differs from the GDPR enforcement process in Europe, where user-initiated regulation of company privacy data protection is the norm. 
%
This top-down privacy law enforcement led by the Chinese government also differs from the decentralized privacy law enforcement in the United States.
}
%
Based upon the laws, other government agencies, such as the Ministry of Industry and Information Technology (MIIT)\ignore{ and the Cyberspace Administration of China (CAC)}, may issue provisions (or terms) to address specific details of the general security and privacy principles. 
%
For example, the ``Several Provisions on Regulating the Market Order of Internet Information Services'' (MIIT Order No. 20, 2011)~\cite{miit2011no20}, the ``Provisions on Protecting the Personal Information of Telecommunications and Internet Users'' (MIIT Order No. 24, 2013)~\cite{miit2013no24}, and the ``Provisions on the Scope of Necessary Personal Information for Common Types of Mobile Applications'' (CAC Order No. 14, 2021)~\cite{cac2021no14}. As the provision titles suggest, these provisions specify requirements for protecting the personal information and rights of Internet users including mobile app users. 
%
\ignore{the ``Provisions on Protecting the Personal Information of Telecommunications and Internet Users'' (Order of MIIT, No. 24, 2013)~\cite{} address requirements for telecommunication and Internet service providers. The ``Provisions on the Scope of Necessary Personal Information for Common Types of Mobile Applications'' (2021)~\cite{} define the detailed list of necessary personal information for common types of apps, and information collected beyond this scope may raise privacy alarms.}
%
In addition to the privacy laws/regulations and provisions, government agencies may release privacy guidelines that offer more practical guidance on interpreting or implementing laws and provisions.
%
For example, on December 30, 2019, MIIT issued a privacy guideline in MIIT Secret [2019] No. 191, titled ``Method for Determining Illegal and Improper Collection and Use of Personal Information by Apps'' (\textit{Guideline-2019}).
%
Although the guideline is not legally binding, it has evolved into a de facto standard used by stakeholders to assess privacy violations in apps.
%
Figure~\ref{fig:law-hierarchy} shows the relationship between privacy laws, provisions, and guidelines. 

\begin{figure}[!t]
\centering
\includegraphics[width=5cm]{pictures/law_hierarchy.pdf}
\caption{Hierarchy of privacy laws, provisions, guidelines, and app review specifications}
\label{fig:law-hierarchy} 
\end{figure}

\para{Special Privacy Rectification Campaigns (SPRCs)}
%
% 电信和互联网用户个人信息保护规定, 常见类型移动互联网应用程序必要个人信息范围规定
%
While agencies like MIIT \ignore{and CAC }do respond to and investigate individual complaints and public reports, the predominant focus of their enforcement efforts so far has been on launching \textit{proactive, nation-wide campaigns} based on the privacy laws/regulations, provisions and guidelines, empowered by increased investment in administrative and social resources.
%
Such campaigns are commonly referred to as \textit{Special Privacy Rectification Campaigns} (SPRCs). 
%
In the field of privacy law enforcement on mobile platforms, MIIT, in collaboration with three other government agencies such as the Cyberspace Administration of China (CAC), has initiated four continuous SPRCs that spanned over four years.
%
In October 2019, MIIT launched an SPRC (\textit{SPRC-2019}~\cite{sprc2019}) by issuing an administrative notice to stakeholders aimed at rectifying mobile apps' infringement of users' privacy rights and interests.
%
Later, in August 2020, July 2021, and February 2023, MIIT revitalized the program with another three SPRCs, \textit{SPRC-2020}~\cite{sprc2020}, \textit{SPRC-2021}~\cite{sprc2021}, and \textit{SPRC-2023}~\cite{sprc2023}, respectively, to further enhance the objectives set forth in prior SPRCs.
% https://www.gov.cn/zhengce/zhengceku/2019-11/13/content_5451505.htm， 工业和信息化部关于开展APP侵害用户权益专项整治工作的通知，2019
% https://www.gov.cn/zhengce/zhengceku/2020-08/02/content_5531975.htm，工业和信息化部关于开展纵深推进APP侵害用户权益专项整治行动的通知，2020
% 《工业和信息化部关于开展互联网行业市场秩序专项整治行动的通知》（工信部信管函[2021]165号）
% https://www.gov.cn/zhengce/zhengceku/2023-03/02/content_5744106.htm，工业和信息化部关于进一步提升移动互联网应用服务能力的通知，2023
%
Note that \textit{SPRC-2019} was launched even before the first privacy guideline on mobile apps, \textit{Guideline-2019}, was released, so much of the \textit{SPRC-2019} is based only on high-level laws and provisions. 
%
Also, the newer SPRCs do not disable but rather complement prior SPRCs by addressing a broader scope of problems and by prioritizing the types of privacy violations that warrant more attention.
%
For example, \textit{SPRC-2019} mandates that app developers and distribution platforms (i.e., app stores) detect and rectify eight types of privacy violations related to the collection, use, and sharing of personal information, as well as difficulties in deleting user accounts.
%
While \textit{SPRC-2020} also covers the aforementioned privacy violations, it expands the requirements to include emerging violations (e.g., personalized ads and deceptive privacy practices) and involves new stakeholders, such as third-party SDK developers.

As described in the administrative notices for launching SPRCs, the SPRCs facilitate two types of app privacy review. First, government agencies would proactively perform privacy reviews to identify potential privacy violations in apps already available on app stores, by themselves or by coordinating app privacy certifications services (or certifiers). Second, SPRCs would mandate major app stores to conduct dedicated privacy reviews for newly submitted apps.
%
Typically, third-party privacy certifiers and app stores develop their own sets of app review specifications based on the requirements outlined in the notices of SPRCs, guided by high-level privacy laws and provisions. 
%
Hence, the app privacy review specifications tend to evolve over time and may vary among app stores and privacy certifiers.
%
\ignore{These specifications, although are developed based on privacy laws/regulations, provisions, and guidelines issued by government agencies, tend to evolve over time in response to changes in SPRCs.}
%
If an app is found to have privacy violations, the app provider must rectify the violations; otherwise, there is a risk of the app being delisted or facing fines.
%
\ignore{In the execution of SPRCs, the government agencies would proactively perform technical tests to identify privacy violations, by coordinating third-party testing services on a large number of publicly available apps. For example, \textit{SPRC-2020} targeted to test 400K popular apps within about four months of its launch. Following this, the agencies would request stakeholders to address identified privacy violations and issue delisting warnings or impose penalties on those who fail to remediate.}
%
Notably, SPRCs do not conclude after a single round of the aforementioned rectification steps; instead, they represent a long-term, ongoing activity that has extended over multiple years until now. To date, the agencies have issued warnings through 36 public privacy bulletins on their websites, akin to walls of shame, with each bulletin listing hundreds (or at least tens) of privacy-violating apps. Figure~\ref{fig:timeline} shows the SPRCs and release time of the privacy bulletins. 

\begin{figure}[!t]
\centering
\includegraphics[width=8cm]{pictures/timeline-01.png}
\caption{Timeline of SPRCs and privacy bulletins issued by government agencies. Each circle (\textcolor{red}{\scriptsize\textcircled{}}) represents a bulletin, with the size of the circle indicating the number of reported apps with privacy violations.}
\label{fig:timeline} 
\end{figure}

\ignore{
Given the importance of achieving privacy compliance, it is imperative to conduct a systematic understanding of such an enforcement practice.
%
This is not only crucial for enhancing the current practice by unveiling the interplay of stakeholders, assessing the current status and challenges for achieving genuine privacy compliance, and guiding the next steps of the practice.
%
More importantly, we firmly believe that this particular practice provides us with a window to generate a quicker and more comprehensive understanding of the development trends in privacy compliance, which can potentially inform future privacy enforcement efforts in other regions worldwide.
}

\if0

% 网络安全法 “Chinese Cybersecurity Law”, 
Enforcement of Chinese laws: 
% 工业和信息化部关于开展APP侵害用户权益专项整治工作的通知 依据《网络安全法》、《电信条例》、《规范互联网信息服务市场秩序若干规定》（工业和信息化部令第20号）、《电信和互联网用户个人信息保护规定》（工业和信息化部令第24号）和《移动智能终端应用软件预置和分发管理暂行规定》（工信部信管〔2016〕407号）等法律法规和规范性文件要求，聚焦人民群众反映强烈和社会高度关注的侵犯用户权益行为，重点对以下四个方面8类问题开展规范整治工作。
% No, a notice is not necessarily a campaign. I might have used the term "campaign" in the translation to convey the idea that it's an organized effort or initiative. A notice typically informs or communicates specific information, while a campaign involves a series of coordinated activities with a particular purpose or goal. If the original context specifies a different nature, please provide more details for a more accurate translation.

"Special Rectification Program"

"Notice from the Ministry of Industry and Information Technology on Carrying Out Special Rectification Work for APPs Infringing on User Rights"

% China PIPL 2021

MIIT Privacy Noncompliance Notifications

~\cite{sun2023gdprxiv}

How GDPR, and US federal/state laws are enforced?

history of mobile privacy regulation enforcement in China. 

the distinction between both.

Different from gdpr enforcement that are primarily driven by data subject complaints and online data breach reports, the chinese act represents a paternalistic enforcement campaign that progressively evaluates the privacy compliance of all apps on the market, by coordinating governmental and societal resources.

How the analysis of Chinese law enforcement informs the privacy enforcement of western countries?

%工业和信息化部关于开展纵深推进APP侵害用户权益专项整治行动的通知
\url{https://www.gov.cn/zhengce/zhengceku/2020-08/02/content_5531975.htm}

% 2019年10月23日，工信部发布《关于开展APP侵害用户权益专项整治工作的通知》（工信部信管函〔2019〕337号），决定组织开展APP侵害用户权益专项整治行动工作，并于2019年12月19日与2020年1月9日先后发布《关于侵害用户权益行为的APP（第一批）通报》与《关于侵害用户权益行为的APP（第二批）通报》，进一步落实对应用软件用户权益的保护。

% 工业和信息化部关于开展APP侵害用户权益专项整治工作的通知
\url{https://www.gov.cn/fuwu/2019-11/07/content_5449660.htm}

% 北京市通信管理局通报2023年第四期问题APP
\url{http://www.cww.net.cn/article?id=578291}

% 工业和信息化部关于电信服务质量的通告（2018年第4号）
% 之前的通报侧重于“强行捆绑推广其他应用软件”，“恶意“吸费””，
\url{https://www.miit.gov.cn/jgsj/xgj/wjfb/art/2020/art_2dda72a495f14b0c9919f286d328d3da.html}

%工信部通报32款不良APP：涉及恶意吸费等问题
%《工业和信息化部关于电信服务质量的通告（2016年第3号）》
\url{http://www.cac.gov.cn/2016-08/06/c_1119346784.htm}

% 工信部第一次通报应用；2014 Apr
% 工业和信息化部关于电信服务质量的通告（2014年第2号）
\url{https://www.miit.gov.cn/zwgk/zcwj/wjfb/tg/art/2020/art_a6f0dfd3966742e4a95fd26b710ed437.html}

% 关于电信服务质量的通告 （最早的2008年5月）
\url{https://www.miit.gov.cn/zwgk/zcwj/wjfb/tg/art/2020/art_a0943a4a32b247748bf37b6a44dabae8.html}

% App合规监管背后：监管机构的分工与职责
\url{https://zhuanlan.zhihu.com/p/431139732}

% 《App违法违规收集使用个人信息行为认定方法》《常见类型移动互联网应用程序必要个人信息范围规定》《个人信息保护法》《网络安全法》《电信条例》《电信和互联网用户个人信息保护规定》
\url{http://www.cac.gov.cn/2021-06/11/c_1624994586637626.htm}

\fi
